Efficient Betti Matching Enables Topology-Aware 3D Segmentation via Persistent Homology

In this work, we propose an efficient algorithm for the calculation of the Betti matching, which can be used as a loss function to train topology aware segmentation networks. Betti matching loss builds on techniques from topological data analysis, specifically persistent homology. A major challenge is the computational cost of computing persistence barcodes. In response to this challenge, we propose a new, highly optimized implementation of Betti matching, implemented in C++ together with a python interface, which achieves significant speedups compared to the state-of-the-art implementation Cubical Ripser. We use Betti matching 3D to train segmentation networks with the Betti matching loss and demonstrate improved topological correctness of predicted segmentations across several datasets. The source code is available at https://github.com/nstucki/Betti-Matching-3D.

==> figures/tex/figure-exampleI.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[height=0.6\textwidth]{figures/exampleI/BBBC027-first-link-small.png0251.png}
        \captionsetup{format=centeredMultilineCaption}
        \caption{Segmentation prediction ($\geq$97\% certainty)}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[height=0.6\textwidth]{figures/exampleI/BBBC027-0.97.pdf}
        \captionsetup{format=centeredMultilineCaption}
        \caption{Cubical grid complex representation}
    \end{subfigure}
    \caption{A predicted segmentation superlevel set on the BBBC027 cell datasets that has two connected components and a loop. With persistent homology, we can capture connected components, loops and cavities at different levels of prediction certainty, and observe how the topology changes as we vary the threshold.}
    \label{fig:persistent-homology-bbbc027-intro-example}
\end{figure}

==> figures/tex/figure-exampleIII-gridComplex.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/exampleIII_cubicalGridComplex.pdf}
    \caption{A cubical grid complex consisting of vertices, edges, 2-cubes and 3-cubes}
    \label{fig:cubicalGridComplex}
\end{figure}


==> figures/tex/figure-exampleVII-imagePersistence.tex <==
\begin{figure}
    \centering
    \hfill
    \begin{subfigure}[t]{0.04\textwidth}
    ~\vspace{-1.09cm}
    
    $\mathbf I$ \vspace{1.33cm}
    
    $\mathbf C$

    % $\mathbf C$ \vspace{1.95cm}
    
    % $\mathbf J$
    \end{subfigure}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input1-0.pdf}
        
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison1-0.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison2-0.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input2-0.pdf}
        \caption*{$r=0.1$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input1-1.pdf}
        
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison1-1.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison2-1.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input2-1.pdf}
        \caption*{$r=0.3$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
       \centering
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input1-2.pdf}
        
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison1-2.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison2-2.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input2-2.pdf}
        \caption*{$r=0.5$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input1-3.pdf}
        
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison1-3.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison2-3.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input2-3.pdf}
        \caption*{$r=0.7$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input1-4.pdf}
        
        \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison1-4.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Comparison2-3.pdf}

        % \includegraphics[width=\textwidth]{figures/exampleVII-2D/exampleVII_2D_Input2-3.pdf}
        \caption*{$r=0.9$}
    \end{subfigure}
    \hfill{}

    \caption{Example of image persistence. The homology class represented by the yellow cycle gets born at $r=0.1$ in $\mathbf C$, but only at $r=0.3$ in $\mathbf I$. It continues to live in $\mathbf I$, with a bar $[0.3, 0.9) \in \mathcal B(\mathbf I)$, but dies in $\mathbf C$ at $r=0.5$, with a bar $[0.1, 0.5) \in \mathcal B(\mathbf C)$. The image barcode captures the threshold span where the class is already alive in $\mathbf I$ and still alive in $\mathbf C$, represented by a bar $[0.3, 0.5) \in \mathcal B(\im \Phi)$. The class represented by the orange cycle never lives in $\mathbf C$ and is not part of the image barcode.}
    \label{fig:image-persistence-example}
\end{figure}

